On Testability of First-Order Properties in Bounded-Degree Graphs and Connections to Proximity-Oblivious Testing

We study property testing of properties that are definable in first-order logic (FO) in the bounded-degree graph and relational structure models. We show that any FO property that is defined by a formula with quantifier prefix $\exists^*\forall^*$ is testable (i.e., testable with constant query complexity), while there exists an FO property that is expressible by a formula with quantifier prefix $\forall^*\exists^*$ that is not testable. In the dense graph model, a similar picture is long known (Alon, Fischer, Krivelevich, Szegedy, Combinatorica 2000), despite the very different nature of the two models. In particular, we obtain our lower bound by an FO formula that defines a class of bounded-degree expanders, based on zig-zag products of graphs. We expect this to be of independent interest. We then use our class of FO definable bounded-degree expanders to answer a long-standing open problem for proximity-oblivious testers (POTs). POTs are a class of particularly simple testing algorithms, where a basic test is performed a number of times that may depend on the proximity parameter, but the basic test itself is independent of the proximity parameter. In their seminal work, Goldreich and Ron [STOC 2009; SICOMP 2011] show that the graph properties that are constant-query proximity-oblivious testable in the bounded-degree model are precisely the properties that can be expressed as a generalised subgraph freeness (GSF) property that satisfies the non-propagation condition. It is left open whether the non-propagation condition is necessary. We give a negative answer by showing that our property is a GSF property which is propagating. Hence in particular, our property does not admit a POT. For this result we establish a new connection between FO properties and GSF-local properties via neighbourhood profiles.

==> listOfNotation.tex <==
%General
\glsxtrnewsymbol[description={the set of natural numbers including $0$}]{NN}{$\mathbb{N}$}
\glsxtrnewsymbol[description={the set of all positive natural numbers}]{NNP}{$\Npos$}
%$\Npos:=\mathbb N\setminus\{0\}$
\glsxtrnewsymbol[description={the set $\{0,\dots,n-1\}$}]{[n]}{$[n]$}
%\glsxtrnewsymbol[description={symmetric group on $[n]$}]{Sn}{$\mathcal{S}_n$}
\glsxtrnewsymbol[description={disjoint union}]{DU}{$\sqcup$}
\glsxtrnewsymbol[description={symmetric difference}]{SD}{$\triangle$}
%\glsxtrnewsymbol[description={probability of $A$}]{ }{$\mathbb{P}[A]$}
\glsxtrnewsymbol[description={the neighbourhood of fixed radius $r$ around $x$, up to isomorphism}]{NBI}{$\tau_r(x)$}
%\glsxtrnewsymbol[description={probability of $A$ under condition $B$}]{Prob}{$\mathbb{P}[A\mid B]$}
%\glsxtrnewsymbol[description={expected value of random variable $X$}]{ExV}$\mathbb{E}[X]$}
%TODO o-natation
%\glsxtrnewsymbol[description={non-deterministic polynomial time}]{NP}{NP}
%\glsxtrnewsymbol[description={polynomial space}]{PSPACE}{PSPACE}
\glsxtrnewsymbol[description={asymtotic upper-bounds}]{big-O}{$\mathcal{O}(\cdot), o(\cdot)$}
%\glsxtrnewsymbol[description={aymtotic tight upper-bound}]{little-O}{$$}
%\glsxtrnewsymbol[description={asymtotic  lower-bound}]{big-Omega}{$\Omega(\cdot)$}
%\glsxtrnewsymbol[description={asymtotic strict lower-bound}]{little-Omega}{$\omega(\cdot)$}
%\glsxtrnewsymbol[description={asymtotic strict-upper- and lower-bound}]{theta}{$\Theta(\cdot)$}
%graphs
\glsxtrnewsymbol[description={zig-zag product}]{zz}{$\zigzag$}
%\glsxtrnewsymbol[description={complete graph on $n$ vertices}]{C}{$K_n$}
\glsxtrnewsymbol[description={expansion ratio of $G$}]{exp}{$h(G)$}
\glsxtrnewsymbol[description={edges crossing $S$ and $T$ in $G$}]{croEd}{$\langle S,T\rangle_G$}
%structures, FO
\glsxtrnewsymbol[description={signature}]{s}{$\sigma$}
\glsxtrnewsymbol[description={signature with one binary relation symbol $E$}]{sg}{$\sigma_{\textrm{graph}}$}
\glsxtrnewsymbol[description={degree of vertex $v$ in $G$}]{deg}{$\deg_G(v)$}
\glsxtrnewsymbol[description={distance between two vertices $v$ and $w$ in $A$}]{dist}{$\dist_A(v,w)$}
\glsxtrnewsymbol[description={distance between structure $A$ and property $\classStruc{P}$}]{distSP}{$\dist(A,\classStruc{P})$}
\glsxtrnewsymbol[description={rotation map of $G$}]{rot}{$\rot_{G}$}

\glsxtrnewsymbol[description={the $(u,v)$ entry of the normalised adjacency matrix $M$ of $G$}]{nam}{$M_{u,v}$}

\glsxtrnewsymbol[description={substracture of $A$ induced by $S$}]{induce}{$A[S]$}
\glsxtrnewsymbol[description={the $r$-neighborhood of $a$ in structure $A$}]{rNBH}{$N_r^A(a)$}

\glsxtrnewsymbol[description={arity of relation $R$}]{relation}{$\ar(R)$}
\glsxtrnewsymbol[description={class of graphs of bounded degree $d$}]{CCn}{$\mathcal{C}_d$}
\glsxtrnewsymbol[description={class of $\sigma$-structures of bounded degree $d$}]{Cn}{$\classStruc{C}_{\sigma,d}$}
\glsxtrnewsymbol[description={property defined by formula $\varphi$}]{PPhi}{$\classStruc{P}_\phi$}
%\glsxtrnewsymbol[description={first-order logic}]{FO}{FO}
%\glsxtrnewsymbol[description={conjunctive normal form}]{CNF}{CNF}
%\glsxtrnewsymbol[description={disjunctive normal form}]{DNF}{DNF}
%\glsxtrnewsymbol[description={Gaifman normal form}]{GNF}{GNF}

\glsxtrnewsymbol[description={prefix classes with $i-1$ quantifier alterations}]{PC}{$\Sigma_i$, $\Pi_i$, $\Delta_i$}
\glsxtrnewsymbol[description={is a model of}]{models}{$\models$}
\glsxtrnewsymbol[description={equivalence of FO-formulas}]{equiv}{$\equiv$}
\glsxtrnewsymbol[description={equivalence of FO-formulas on structures of bounded degree $d$}]{dEquiv}{$\equiv_d$}
\glsxtrnewsymbol[description={logical negation, conjunction, disjunction, implication and biimplication}]{l}{$\lnot$, $\land$, $\lor$, $\rightarrow$, $\leftrightarrow$}
\glsxtrnewsymbol[description={existential and universal quantifier}]{quant}{$\exists$, $\forall$}
%property testing

\glsxtrnewsymbol[description={answer to query $q$ to structure $\mathcal{A}$}]{query}{$\operatorname{ans}_{\mathcal{A}}(q)$}
\glsxtrnewsymbol[description={binary relation symbols for $i,j\in [D]^2$ and $k\in ([D]^2)^2$}]{binary}{$E_{i,j}$, $F_{k}$, $R$, $L_k$}

\glsxtrnewsymbol[description={underlying graph of a model $\struc{A}$ of $\varphi_{\zigzag}$}]{underlying}{$\underlyingGraph{\struc{A}}$}

\glsxtrnewsymbol[description={the formula definded in Section \ref{sec: definitionFormula} whose underlying graphs are expanders }]{expander}{$\varphi_{\zigzag}$}


\glsxtrnewsymbol[description={a set of models of some sentence in $\Sigma_2$ }]{modelset}{$\mathfrak{M}$}


\glsxtrnewsymbol[description={a maximal set of pairwise non-isomorphic structures in $\classStruc{C}_{\sigma,d}$}]{maximal}{$\mathfrak{H}$}


\glsxtrnewsymbol[description={a conjunction of atomic (resp. negated) formulas containing both variables from tuples $\overline{x}$ and $\overline{y}$}]{positive}{$\operatorname{pos}^i(\overline{x},\overline{y}),\operatorname{neg}^i(\overline{x},\overline{y})$}

\glsxtrnewsymbol[description={the number of maximal $i$-cliques containing $v$}]{maxcl}{$\maxcl^G(v,i)$}
%$\maxcl^G(v,i):=|\{K\in \setOfMaxCliques\mid |K|=i,v\in K\}|$  is .
\glsxtrnewsymbol[description={the set of maximal cliques in $G$}]{setclique}{$\setOfMaxCliques$}
%et $\setOfMaxCliques$ be 
\glsxtrnewsymbol[description={the $r$-type distribution of  $\struc{A}$}]{rho}{$\rho_{\struc{A},r}$}
%et $\setOfMaxCliques$ be 

\glsxtrnewsymbol[description={the sampling distance of depth $r$ between two $\sigma$-structures $\struc{A}$ and $\struc{B}$ }]{samplingdist}{$\delta_{\odot}^r(\struc{A},\struc{B})$}


\glsxtrnewsymbol[description={Hanf normal form}]{HNF}{HNF}
\glsxtrnewsymbol[description={proximity oblivious tester}]{POT}{POT}
\glsxtrnewsymbol[description={generalised subgraph freeness}]{GSF}{GSF}



%
%\glsxtrnewsymbol[description={a conjunction of atomic (resp. negated) formulas containing both variables from tuples $\overline{x}$ and $\overline{y}$}]{negative}{$\operatorname{neg}^i(\overline{x},\overline{y})$}
%
%$\operatorname{neg}^i(\overline{x},\overline{y})$ is a conjunction of negated atomic formulas containing both variables from $\overline{x}$ and $\overline{y}$ and $\operatorname{pos}^i(\overline{x},\overline{y})$ is a conjunction of atomic formulas containing both variables from $\overline{x}$ and $\overline{y}$. 

